Non-Autoregressive Neural Dialogue Generation

Maximum Mutual information (MMI), which models the bidirectional dependency between responses ($y$) and contexts ($x$), i.e., the forward probability $\log p(y|x)$ and the backward probability $\log p(x|y)$, has been widely used as the objective in the \sts model to address the dull-response issue in open-domain dialog generation. Unfortunately, under the framework of the \sts model, direct decoding from $\log p(y|x) + \log p(x|y)$ is infeasible since the second part (i.e., $p(x|y)$) requires the completion of target generation before it can be computed, and the search space for $y$ is enormous. Empirically, an N-best list is first generated given $p(y|x)$, and $p(x|y)$ is then used to rerank the N-best list, which inevitably results in non-globally-optimal solutions. In this paper, we propose to use non-autoregressive (non-AR) generation model to address this non-global optimality issue. Since target tokens are generated independently in non-AR generation, $p(x|y)$ for each target word can be computed as soon as it's generated, and does not have to wait for the completion of the whole sequence. This naturally resolves the non-global optimal issue in decoding. Experimental results demonstrate that the proposed non-AR strategy produces more diverse, coherent, and appropriate responses, yielding substantive gains in BLEU scores and in human evaluations.

==> case_study.tex <==
\begin{table*}
\small
\begin{tabular}{ll}\hline
\textsc{example1} & [john scottsdale] \begin{tiny}PER: PHYS-1\end{tiny} is on the front lines in [iraq]\begin{tiny}GPE: PHYS-1\end{tiny} .  \\\hline
\textsc{MRT} & [john scottsdale] \begin{tiny}PER\end{tiny} is on the front lines in [iraq]\begin{tiny}GPE\end{tiny} .   \\\hline
\textsc{Multi-QA} & [john scottsdale] \begin{tiny}PER: PHYS-1\end{tiny} is on the front lines in [iraq]\begin{tiny}GPE: PHYS-1\end{tiny} .  \\\hline
\hline
\textsc{example2} & The [men]\begin{tiny} PER: ART-1\end{tiny} held on the sinking [vessel]\begin{tiny} VEH: ART-1\end{tiny}  until the [passenger]\begin{tiny} PER: ART-2\end{tiny}  [ship]\begin{tiny} VEH: ART-2\end{tiny}  was able to reach them. \\\hline 
\textsc{MRT} & The [men]\begin{tiny} PER: ART-1\end{tiny} held on the sinking [vessel]\begin{tiny} VEH: ART-1\end{tiny} until  the [passenger]\begin{tiny}PER\end{tiny} ship was able to reach them. \\\hline 
\textsc{Multi-QA} & The [men]\begin{tiny} PER: ART-1\end{tiny} held on the  sinking [vessel]\begin{tiny} VEH: ART-1\end{tiny}  until the [passenger]\begin{tiny} PER: ART-2\end{tiny}  [ship]\begin{tiny} VEH: ART-2\end{tiny} was able to reach them. \\\hline 
\end{tabular}
\caption{Comparing the multi-turn QA model with MRT \cite{sun2018extracting}.}
\label{case}
\end{table*}

==> exp-result.tex <==
\begin{table*}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{4pt}
% \resizebox{\linewidth}{28mm}{
\begin{tabular}{l@{\hspace{0.3cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}}
\toprule
 & \multicolumn{3}{c}{\bf CTB5}& \multicolumn{3}{c}{\bf CTB6}& \multicolumn{3}{c}{\bf UD1.4} \\\hline
%\multicolumn{4}{c}{Chinese CTB5}\\\hline
{\bf Model} & {\bf Prec.} & {\bf Rec.} & {\bf F1} & {\bf Prec.} & {\bf Rec.} & {\bf F1} & {\bf Prec.} & {\bf Rec.} & {\bf F1}  \\
\midrule
- \cite{} &93.68&94.47&94.07 &-&-&90.81 &89.28&89.54&89.41\\
-\cite{} &93.95&94.81&94.38&-&-&-&89.67&89.86&89.75\\
-\cite{}  & 94.77& 95.51& 95.14& 92.00& 90.86&91.43&90.47&89.70& 90.09 \\
-\cite{}& 95.86 & 96.26 & {\bf 96.06} & 94.91 & 94.63 & {\bf 94.77} & 95.42 & 94.17 & {\bf 94.79}\\
\hline
% BERT+WeightCE & 96.45 & 96.41 & 96.43 & 95.34 & 96.22 & 95.78 & 96.09 & 97.08 & 96.58  \\
%  &  &  & (+0.37) &  &  & (+1.01) &  &  & (+1.79)  \\\hline
- & 96.11 & 97.42 &  96.76& 95.80 & 95.08 &  95.44 & 96.33 & 95.85 & 96.81 \\
 & & &  (+0.70)&  &  &  (+0.67) &  &  & (+2.02) \\\hline
- & 96.77  & 98.87 & 97.81& 94.08 & 96.12 & 95.09  & 96.10 & 97.79 & 96.94 \\
&  &  & (+1.75)&  &  & (+0.32)  &  &  & (+2.15) \\\hline
- & 97.10 &98.75& \textbf{97.92} & 96.29& 96.85& \textbf{96.57}  & 96.24 & 97.73 & \textbf{96.98} \\
 &  && \textbf{(+1.86)} & & & \textbf{(+1.80)}  & &  & \textbf{(+2.19)}
\\
\bottomrule\hline

\end{tabular}
%}
\caption{Experimental results on WMT2014 En-De, WMT16 En-De and  }
\label{tab:pos_result}
\vskip -0.15in
\end{table*}
